Knowledge Graphs Meet Multi-Modal Learning: A Comprehensive Survey

Knowledge Graphs (KGs) play a pivotal role in advancing various AI applications, with the semantic web community's exploration into multi-modal dimensions unlocking new avenues for innovation. In this survey, we carefully review over 300 articles, focusing on KG-aware research in two principal aspects: KG-driven Multi-Modal (KG4MM) learning, where KGs support multi-modal tasks, and Multi-Modal Knowledge Graph (MM4KG), which extends KG studies into the MMKG realm. We begin by defining KGs and MMKGs, then explore their construction progress. Our review includes two primary task categories: KG-aware multi-modal learning tasks, such as Image Classification and Visual Question Answering, and intrinsic MMKG tasks like Multi-modal Knowledge Graph Completion and Entity Alignment, highlighting specific research trajectories. For most of these tasks, we provide definitions, evaluation benchmarks, and additionally outline essential insights for conducting relevant research. Finally, we discuss current challenges and identify emerging trends, such as progress in Large Language Modeling and Multi-modal Pre-training strategies. This survey aims to serve as a comprehensive reference for researchers already involved in or considering delving into KG and multi-modal learning research, offering insights into the evolving landscape of MMKG research and supporting future work.

==> 0-author.tex <==
% First author
%
% Options: Use if required
% eg: \author[1,3]{Author Name}[type=editor,
%       style=chinese,
%       auid=000,
%       bioid=1,
%       prefix=Sir,
%       orcid=0000-0000-0000-0000,
%       facebook=<facebook id>,
%       twitter=<twitter id>,
%       linkedin=<linkedin id>,
%       gplus=<gplus id>]

%\author[1,2]{Zhuo Chen}[orcid=0000-0001-9991-6892]
%\author[1]{Yichi Zhang}[orcid=0009-0007-4046-1003]
%\author[3]{Yuxia Geng}[orcid=0000-0002-2461-2613]
%\author[1]{Lingbing Guo}[orcid=0000-0002-8589-276X]
%\author[1]{Yushan Zhu}[orcid=0000-0001-9991-6892]
%\author[1,2]{Yajing Xu}[orcid=0000-0001-9991-6892]
%\author[1]{Yin Fang}[orcid=0000-0001-9538-848X]
%\author[4]{Yufeng Huang}[orcid=0000-0001-7110-9298]
%\author[1,2]{Jiaoyan Chen}[orcid=0000-0001-9991-6892]
%\author[4,2,1]{Wen Zhang}[orcid=0000-0001-8429-9326]

\author[1,2]{Zhuo Chen}
\author[1]{Yichi Zhang}
\author[3]{Yuxia Geng}
\author[1]{Lingbing Guo}
\author[1]{Yin Fang}
\author[1]{Xiang Chen}
\author[1]{Yushan Zhu}
\author[5]{Jiaqi Li}
\author[6]{Qian Li}
\author[7]{Xiaoze Liu}
\author[4]{Yufeng Huang}
\author[8,9]{Jiaoyan Chen}
\author[10]{Yangning Li}
% \author[1,2]{Yajing Xu}
\author[11]{Bolin Zhu}
\author[12]{Jeff Z. Pan}
% \author[4,2]{Ningyu Zhang}
% \author[13]{Zequn Sun}
% \author[5]{Meng Wang}
% \author[13]{Haofen Wang}
% \author[5]{Guilin Qi}
% \author[13]{Wei Hu}
\author[1,2]{Huajun Chen}
\author[4,1,2]{Wen Zhang}[orcid=0000-0001-8429-9326]

% Corresponding author indication
\cormark[1]

%% Footnote of the first author
%\fnmark[<footnote mark no>]

% Email id of the first author
\ead{zhang.wen@zju.edu.cn}


%% URL of the first author
%\ead[url]{<URL>}

%% Credit authorship
%% eg: \credit{Conceptualization of this study, Methodology, Software}
%\credit{<Credit authorship details>}

% Address/affiliation


\affiliation[a]{
organization={College of Computer Science},
organization={Zhejiang University},
city={Hangzhou},
state={Zhejiang},
country={China}}
\affiliation[b]{
organization={Donghai laboratory},
city={Zhoushan},
state={Zhejiang},
country={China}}
\affiliation[c]{
organization={School of Computer Science},
organization={Hangzhou Dianzi University},
city={Hangzhou},
state={Zhejiang},
country={China}}
\affiliation[d]{
organization={School of Software Technology},
organization={Zhejiang University},
city={Ningbo},
state={Zhejiang},
country={China}}
\affiliation[e]{
organization={School of Computer Science and Engineering},
organization={Southeast University},
city={Nanjing},
state={Jiangsu},
country={China}}
\affiliation[g]{
organization={Baidu},
city={Beijing},
state={Beijing},
country={China}}
\affiliation[f]{
organization={Elmore Family School of Electrical and Computer Engineering},
organization={ Purdue University},
city={West Lafayette},
state={Indiana},
country={USA}}
\affiliation[h]{
organization={Department of Computer Science},
organization={The University of Manchester},
city={Manchester},
country={United Kingdom}}
\affiliation[i]{
organization={Department of Computer Science},
organization={The University of Oxford},
city={Oxford},
country={United Kingdom}}
\affiliation[j]{
organization={Shenzhen International Graduate School},
organization={Tsinghua University},
city={Shenzhen},
country={China}}
\affiliation[k]{
organization={College of Computer Science},
organization={Fudan University},
city={shanghai},
state={Shanghai},
country={China}}
\affiliation[l]{
organization={School of Informatics},
organization={The University of Edinburgh},
city={Edinburgh},
country={United Kingdom}}
\affiliation[m]{
organization={College of Computer Science},
organization={Nanjing University},
city={Nanjing},
state={Jiangsu},
country={China}}
% \affiliation[m]{
% organization={School of Computer Science and Engineering},
% organization={Tongji University},
% city={Shanghai},
% state={Jiangsu},
% country={China}}

% Corresponding author text
\cortext[1]{Corresponding author}

==> 4.0-kgr.tex <==
\subsection{KG Representation Learning}\label{sec:kgrl}

\textbf{\textit{(\rmnum{1})} GNN-based methods} ...

\textbf{\textit{(\rmnum{2})} KGE-based methods}...

\textbf{\textit{(\rmnum{3})} Retrieval-based methods} ..

\textbf{\textit{(\rmnum{5})} Serialization-based methods} ..

\textbf{\textit{(\rmnum{4})} Semantic parsing-based methods} ..







==> 6-indus.tex <==
% \section{Industry Application}\label{sec:indus}

% \input{6.1-kgmm-indus}
% \input{6.2-mmkg-indus}


==> 7.2-ai4sci.tex <==
\subsection{AI for Science}

% 已有方向如何延续，有哪些新的大方向。参考NMI
% Multimodal Biological Knowledge Graph Completion via Triple Co-attention Mechanism
% Multi-modal protein knowledge graph construction and applications (student abstract)
% Ai4Science 方向有哪些是多模态KG或者说KG能够帮助的，Ai4Science 中的多模态场景是否能有KG发挥作用？
% 中医药
% \fy{
% \begin{itemize}
%     \item Challenges and Issues: Detailed discussion on the main problems and challenges currently faced in the field of ... (shortcomings on methods or settings).
%     \item Future Directions: Discussion on potential future research directions and further developments possibilities in ....
%     \item what can MMKG or KG do for Science.
%     \item multi-modal Science KG
%     \item  multi-modal learning \& KG for Science  
% \end{itemize}
% }


Despite the vast potential of biological MMKGs in drug discovery, several challenges exist. 
One of the primary hurdles is the issue of data heterogeneity and quality, which demands meticulous integration and standardization of data from diverse sources.
Another major challenge lies in the choice of knowledge representation within these MMKGs. The ideal representation would capture the intricate details of drug discovery objects and relationships, such as the various protein isoforms produced from a single gene and their complex interactions within cellular environments. However, achieving this level of detail is often hindered by practical constraints like cost and technology limitations. 
Furthermore, specific data sources may impose additional limitations based on their existing information structures. As such, the chosen knowledge representation in MMKGs often has to strike a balance between desired granularity and practical feasibility, reflecting both the current state of scientific knowledge and the inherent limitations of data sources. This balancing act poses a significant challenge and indicates the need for ongoing efforts to refine and expand the scope and depth of MMKGs in the field of drug discovery.

==> tab/kgmm-tree.tex <==
\tikzstyle{leaf}=[mybox,minimum height=1.5em,
fill=hidden-orange!60, text width=20em,  text=black,align=left,font=\scriptsize,
inner xsep=2pt,
inner ysep=4pt,
]

\begin{figure*}[tp]
  \centering
  \resizebox{\textwidth}{!}{
    \begin{forest}
      forked edges,
      for tree={
          grow=east,
          reversed=true,%increase counter-clockwise
          anchor=base west,
          parent anchor=east,
          child anchor=west,
          base=center,
          font=\scriptsize,
          rectangle,
          draw=hiddendraw,
          rounded corners,align=left,
          minimum width=6em,
            edge+={darkgray, line width=1pt},
            %  l sep+=2.5pt,
            %  s sep+=-5pt,
            s sep=3pt,
            inner xsep=2pt,
            inner ysep=3pt,
            % inner xsep=2pt,
            % inner ysep=5pt,
            %align=center,
            ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
          },
      % where level=1{text width=3em,font=\scriptsize,}{},
      % where level=2{text width=4.5em,font=\scriptsize,}{},
        where level=1{text width=4.8em,font=\scriptsize,align=center}{},
        where level=2{text width=7.2em,font=\scriptsize,align=center}{},
        where level=3{text width=4.0em,font=\scriptsize,align=center}{},
        [
            \quad (\S \ref{sec:kg4mmtask}) KG-driven Multi-modal Learning \quad, ver,font=\small
            % [
            %     (\S \ref{sec:kgrl}) KG \\ Representation   
            %     [ 
            %         todo~ {,}
            %         todo~ {,}
            %         todo~ {,}
            %         todo~ {,}\\
            %         todo~ 
            %         ,leaf,text width=41.9em
            %     ]
            % ]
            [
                (\S \ref{sec:kggen}) Content \\ Generation
                [ 
                    (\S \ref{sec:kgic})  Image \\ Captioning
                    [ 
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ 
                        ,leaf,text width=33em
                    ]
                ]
                [ 
                    (\S \ref{sec:kgvs}) Visual \\ Storytelling
                    [ 
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ 
                        ,leaf,text width=33em
                    ]
                ]
                [ 
                    (\S \ref{sec:kgctg}) Text-to-\\Image Generation
                    [ 
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ 
                        ,leaf,text width=33em
                    ]
                ]
                [ 
                    (\S \ref{sec:kgsgg}) Scene Graph \\Generation
                    [ 
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ 
                        ,leaf,text width=33em
                    ]
                ]
            ]
            [
                (\S \ref{sec:kgr})Reasoning\\\&Understanding
                [ 
                    (\S \ref{sec:kgvqa}) Visual \\  Question Answering
                    [ 
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ 
                        ,leaf,text width=33em
                    ]
                ]
                % [ 
                %     (\S \ref{sec:kgvr}) Visual Com-\\monsense Reasoning
                %     [ 
                %         todo~ {,}
                %         todo~ {,}
                %         todo~ {,}
                %         todo~ {,}
                %         todo~ 
                %         ,leaf,text width=33em
                %     ]
                % ]
                [ 
                    (\S \ref{sec:kgvd}) Visual \\ Dialog
                    [ 
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ 
                        ,leaf,text width=33em
                    ]
                ]
            ]
            [
                (\S \ref{sec:kgcls}) \\Classification  
                [ 
                    (\S \ref{sec:kgimgc}) Image \\ Classification
                    [ 
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ 
                        ,leaf,text width=33em
                    ]
                ]
                % [ 
                %     (\S \ref{sec:kgfnd}) Fake News \\ Detection
                %     [ 
                %         todo~ {,}
                %         todo~ {,}
                %         todo~ {,}
                %         todo~ {,}
                %         todo~ 
                %         ,leaf,text width=33em
                %     ]
                % ]
                % [ 
                %     (\S \ref{sec:kgmc}) Movie \\ Classification
                %     [ 
                %         todo~ {,}
                %         todo~ {,}
                %         todo~ {,}
                %         todo~ {,}
                %         todo~ 
                %         ,leaf,text width=33em
                %     ]
                % ]
            ]
            [
                (\S \ref{sec:kgret}) Retrieval 
                [ 
                    (\S \ref{sec:kgcmr}) Cross-Modal \\ Retrieval
                    [ 
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ 
                        ,leaf,text width=33em
                    ]
                ]
                [ 
                    (\S \ref{sec:kgvre}) Visual Refer-\\ring Expressions
                    [ 
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ 
                        ,leaf,text width=33em
                    ]
                ]
                [ 
                    (\S \ref{sec:kgrt}) Retrieval-\\augmented Tasks
                    [ 
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ {,}
                        todo~ 
                        ,leaf,text width=33em
                    ]
                ]
            ]
            [
                (\S \ref{sec:kgplm}) \\ Pre-training 
                [ 
                    todo~ {,}
                    todo~ {,}
                    todo~ {,}
                    todo~ {,}
                    todo~ 
                    ,leaf,text width=41.9em
                ]
            ]
            [
                (\S \ref{sec:indus-mm4kg}) Industry \\ Application
                [
                    todo~ {,}
                    todo~ {,}
                    todo~ {,}
                    todo~ {,}\\
                    todo~ 
                    ,leaf,text width=41.9em
                ]
            ]
        ]
\end{forest}
}
\caption{ Taxonomy of the KG-driven Multi-modal Learning Realm.}
\label{fig:taxonomy_of_kgmm}
\end{figure*}

==> tab/mmea-fb_db_yg.tex <==
\begin{table*}[ht]\centering
    \setlength{\tabcolsep}{1.3mm}{
        \centering
%    \footnotesize
	% \tabcolsep=0.3cm
    \renewcommand\arraystretch{1.0}
        \caption{Comparison of MMEA results on the FB15K-DB15K\ /\ FB15K-YG15K datasets
    }
    \label{tab:mmea-fbdbyg}
\begin{tabular}{l|rrrrr|rrrrr}
    \Xhline{1px} \multicolumn{1}{c|}{\multirow{2}{*}{{Method}}} & \multicolumn{5}{c|}{{FB15K-DB15K}} & \multicolumn{5}{c}{{FB15K-YG15K}} \\ %\cline{2-11} 
     & {H@1}$\uparrow$  & {H@5}$\uparrow$  & {H@10}$\uparrow$  & {MR}$\downarrow$  & {MRR}$\uparrow$  & {H@1}$\uparrow$  & {H@5}$\uparrow$  & {H@10}$\uparrow$  & {MR}$\downarrow$  & {MRR}$\uparrow$  \\ \Xhline{1px}
    MTransE~\cite{MTransE17} & 0.4 & 1.4 & 2.5 & 1239.5 & 0.014 & 0.3 & 1.0 & 1.8 & 1183.3 & 0.011 \\
    IPTransE~\cite{IPTransE17} & 4.0 & 11.2 & 17.3 & 387.5 & 0.086 & 3.1 & 9.5 & 14.4 & 522.2 & 0.070 \\
    GCN-Align~\cite{GCN-Align18} & 7.1 & 16.5 & 22.4 & 304.5 & 0.106 & 5.0 & 12.9 & 18.1 & 478.2 & 0.094 \\
    BootEA~\cite{BootEA18} & 32.3 & 49.9 & 57.9 & 205.5 & 0.410 & 23.4 & 37.4 & 44.5 & 272.1 & 0.307 \\
    SEA~\cite{SEA19} & 17.0 & 33.5 & 42.5 & 191.9 & 0.255 & 14.1 & 28.7 & 37.1 & 207.2 & 0.218 \\
    IMUSE~\cite{IMUSE19} & 17.6 & 34.7 & 43.5 & 182.8 & 0.264 & 8.1 & 19.2 & 25.7 & 397.6 & 0.142 \\
    HyperKA~\cite{HyperKA20} & 13.7 & 24.9 & 30.7 & 712.2 & 0.195 & 16.9 & 29.5 & 34.9 & 738.0 & 0.232 \\
    % RAGA~\cite{} & 6.1 & 11.5 & 15.0 & 1519.0 & 0.092 & 5.5 & 10.3 & 12.8 & 1337.8 & 0.082 \\
    % RAC~\cite{} & 20.3 & 37.0 & 43.2 & 453.3 & 0.281 & 15.1 & 28.1 & 34.5 & 501.8 & 0.216 \\
    DualAMN~\cite{DualAMN21}& 55.0 & 71.4 & 77.1 & 166.6 & 0.627 & 51.6 & 68.3 & 74.4 & 115.1 & 0.594 \\
    \Xhline{1px}
    PoE~\cite{DBLP:conf/esws/LiuLGNOR19} & 12.0 & - & 25.6 & - & 0.167 & 10.9 & - & 24.1 & - & 0.154 \\
    MMEA~\cite{DBLP:conf/ksem/ChenLWXWC20} & 26.5 & 45.1 & 54.1 & 124.8 & 0.357 & 23.4 & 39.8 & 48.0 & 147.4 & 0.317 \\
    ACK-MMEA~\cite{ACKMMEA} & 30.4 & - & 54.9 & - & 0.387 & 28.9 & - & 49.6 & - & 0.360 \\
    MCLEA~\cite{DBLP:conf/coling/LinZWSW022} & 44.5 & - & 70.5 & - & 0.534 & 38.8 & - & 64.1 & - & 0.474 \\
    EVA~\cite{DBLP:conf/aaai/0001CRC21} & 55.6 & 66.6 & 71.6 & 140.0 & 0.609 & 10.3 & 21.7 & 27.8 & 616.8 & 0.164 \\
    MEAformer~\cite{chen2023meaformer} & 57.8 & - & 81.2 & - & 0.661 & 44.4 & - & 69.2 & - & 0.529 \\
    MSNEA~\cite{DBLP:conf/kdd/ChenL00WYC22} & 65.3 & 76.8 & 81.2 & 54.0 & 0.708 & 44.3 & 62.6 & 69.8 & 85.1 & 0.529 \\ 
    PathFusion~\cite{zhu2023universal} & 87.7 & 93.0 & 94.5 & 22.7 & 0.902 & 80.5 & 88.0 & 90.1 & 36.4 & 0.839 \\ 
    \Xhline{1px}
    \end{tabular}}
\end{table*}
